Stronger generalization bounds for deep nets via a compression approach

Deep nets generalize well despite having more parameters than the number of training samples. Recent works try to give an explanation using PAC-Bayes and Margin-based analyses, but do not as yet result in sample complexity bounds better than naive parameter counting. The current paper shows generalization bounds that're orders of magnitude better in practice. These rely upon new succinct reparametrizations of the trained net --- a compression that is explicit and efficient. These yield generalization bounds via a simple compression-based framework introduced here. Our results also provide some theoretical justification for widespread empirical success in compressing deep nets. Analysis of correctness of our compression relies upon some newly identified \textquotedblleft noise stability\textquotedblright properties of trained deep nets, which are also experimentally verified. The study of these properties and resulting generalization bounds are also extended to convolutional nets, which had eluded earlier attempts on proving generalization.

==> experimentsmain.tex <==
\section{Empirical Evaluation}
\label{sec:experiments}
We study noise stability properties (defined in Section~\ref{sec:stability}) of an actual trained deep net, and compute a generalization bound from Theorem~\ref{thm:convolution:main}. Experiments were performed by training a VGG-19 architecture \cite{simonyan2014very}  for multi-class classification task on CIFAR-10 dataset. Optimization used SGD with mini-batch size 128, weight decay 5e-4,  momentum $0.9$ and initial learning rate $0.05$, but decayed by factor 2 every 30 epochs.  Drop-out was used in fully-connected layers. We trained the network for 299 epochs and the final network achieved $100\%$ training and $92.45\%$ validation accuracy.

%Please see Section~\ref{exp:verify_assumption} for details on the 
Our estimate of the sample complexity bound used exact computation of norms of weight matrices (or tensors) in all bounds($||A||_{1,\infty}, ||A||_{1,2}, ||A||_{2}, ||A||_F$). Like previous bounds in generalization theory, ours also depend upon nuisance parameters like  depth $d$, logarithm of $h$, etc.  which probably are an artifact of the proof. These are ignored in the computation (also in computing earlier bounds) for simplicity. 
  Even the generalization based on parameter counting arguments does have an extra dependence on depth~\cite{bartlett2017}. A recent work, \citet{golowich2017size} showed that many such depth dependencies can be improved. 



\subsection{Empirical investigation of noise stability properties}\label{exp:verify_assumption}
Section \ref{sec:stability}  identifies four properties in the networks that contribute to noise-stability: layer cushion, interlayer cushion, contraction, interlayer smoothness. Figure~\ref{fig:verify} plots the distribution of  over different data points in the training set and compares  to a Gaussian random network and then scaled properly. The layer cushion, which quantifies its noise stability, is drastically improved during the training, especially for the higher layers ($8$ and higher) where most parameters live. Moreover, we observe that interlayer cushion, activation contraction and interlayer smoothness behave nicely even after training.  These plots suggest that the  driver of the generalization pehnomenon is layer cushion.  The other properties are  being maintained in the network and prevent the network from falling prey to pessimistic assumptions that causes the other older generalization bounds to be very high.
The assumptions made in section~\ref{sec:stability} (also in~\ref{conditions}) are verified on the VGG-19 net in appendix~\ref{appdix:verification} by histograming the distribution of layer cushion, interlayer cushion, contraction, interlayer smoothness, and well-distributedness of the Jacobians of each layer of the net on each data point in the training set. Some examples are shown in Figure~\ref{fig:verify}.
%Our assumptions are empirically ceritified. 
% Our assumptions are empirically ceritified. Overall, later layers of the network (from layer 8 to layer 16) have better parameters, indicating better compressibility than the earlier ones.

\begin{figure}[ht]
	\centering
	\includegraphics[width=8cm]{figures/pannels.pdf}
	\caption{this noise gets attenuated as it propagates up to higher layers}
	\label{fig:noise_decay}
	\vspace{-0.5cm}
\end{figure}

\subsection{Correlation to generalization error}
%We show our bound is significantly tighter than other suggested generalization bounds. However, a capacity measure is more informative if it correlates with generalization error, i.e. models that have lower capacity measures generalize better. If a capacity measure correlates with generalization, then perhaps explicit or implicit regularization of that measure improves the generalization. 
We evaluate our generalization bound during the training, see Figure~\ref{fig:comparison}, Right. % of VGG-19 on CIFAR-10. An interesting observation is that 
After 120 epochs, the training error is almost zero but the test error continues to improve in later epochs. Our generalization bound continues to improve, though not to the same level. Thus our generalization bound captures part of generalization phenomenon, not all.
Still, this suggests that SGD somehow improves our generalization measure implicitly. Making this rigorous is a good topic for further research.
 %This is clearly due to implicit regularization of the optimizaiton method. 
%The right pannel in Figure~\ref{fig:comparison} shows the generalization error after epoch 120 together with our bound (rescaled to fit in the plot). The figure suggests our measure correlates with better generalization and that the optimization algorithm (SGD) is implicitly regularizating our measure. This of course does not mean that SGD directly optimzes this measure but it could minimize a measure that is well-correlated with ours. This finding indicates that properties identified in the newtork to bound the generalization, are indeed relavant.
\iffalse 

 our suggested generalization bound against other proposed bounds and the number of parameters in the network. We Further show that our bound correlates with better generalization and is being implicitly minimized during the optimization. Finally, we look into individual properties of the network that allow noise stability and we compare them to those in a random network.
\fi 





%\subsection{Experimental Setup}


\subsection{Comparison to other generalization bounds}\label{sec:comparison}
Figure~\ref{fig:comparison} compares our proposed bound to other neural-net generalization bounds on the VGG-19 net and compares to naive VC dimension bound (which of course is too pessimistic).  All previous generalization bounds are orders of magnitude worse than ours; the closest one is spectral norms times average $\ell_{1,2}$ of the layers \citet{bartlett2017spectrally} which is still about $10^{15}$, far greater than VC dimension. (As mentioned we're ignoring nuisance factors like depth and $\log h$ which make the comparision to VC dimension a bit unfair, but the comparison to previous bounds is fair.)
%On the contrast, our capacity measure is significantly lower than other proposed ones and is even smaller than the number of parameters (ignoring depth and log factors). This is however, should 
This should not be surprising as all other bounds are based on product of norms which is pessimistic (see note at the start of Section~\ref{sec:stability}) which we avoid due to the  noise stability analysis.

Table~\ref{table:compress1} shows the compressibility of various layers according to the bounds given by our theorem. Again, this is a qualitative due to ignoring nuisance factors, but it gives an idea of which layers are important in the calculation.
%In contrast, we identified properties of networks trained on real data that allows our bound to instead depends on the magnitude of the output of the network which epirically does not depend on the depth for network.

\begin{figure}[H]
	
	\centering
	\begin{subfigure}{0.23\textwidth}
		\includegraphics[width=3.8cm,height=3.5cm]{compare.pdf}
	\end{subfigure}
	~
	\begin{subfigure}{0.2\textwidth}
		\vspace{-0.3cm}
		\includegraphics[width=3.9cm]{generalization.pdf}
	\end{subfigure}
	\vspace{-0.2cm}
	\caption{ Left) \small Comparing neural net genrealization bounds. $\ell_{1,\infty}:$ $\frac{1}{\gamma^2}\prod_{i=1}^d||A^i||_{1,\infty}$~\cite{bartlett2002rademacher}\\
		Frobenius: $\frac{1}{\gamma^2}\prod_{i=1}^d||A^i||_F^2$~\cite{NeyTomSre15},\\
		spec $\ell_{1,2}$: $\frac{1}{\gamma^2}\prod_{i=1}^d||A_i||_2^2\sum_{i=1}^d\frac{||A^i||_{1,2}^2}{||A^i||_2^2}$ \cite{bartlett2017spectrally}\\
		spec-fro: $\frac{1}{\gamma^2}\prod_{i=1}^d||A^i||_2^2\sum_{i=1}^dh_i\frac{||A^i||_F^2}{||A^i||_2^2}$~\cite{neyshabur2017pac}\\
		ours: $\frac{1}{\gamma^2}\max_{x\in S}||f(x)||_2^2\sum_{i=1}^d\frac{\beta^2 c_i^2 \lceil\kappa/s\rceil^2 }{\mu_i^2\mu_{i\rightarrow}^2}$\\
		Right) Comparing our bound to empirical generalization error during training. Our bound is rescaled to be within the same range as the generalization error.}
	\label{fig:comparison}
	\vspace{-0.5cm}
\end{figure}
 %One possible interesting research question is whether or not regularizing our measure can help networks generalize better.

\begin{table}[H]
\centering
 \begin{tabular}{c | c c c} 

 layer & $  \frac{c_i^2\beta_i^2\lceil\kappa_i/s_i\rceil^2}{\mu_i^2\mu_{i\rightarrow}^2} $ &  actual \# param & compression ($\%$) \\ [0.5ex] 
 \hline
  1 & 1644.87 & 1728 & 95.18 \\ 
  \hline
 4 & 644654.14 & 147456 & 437.18\\
 \hline
  6 & 3457882.42 & 589824 & 586.25\\
  \hline
 9 & 36920.60 & 1179648 & 3.129 \\
  \hline 
 12 & 22735.09  & 2359296 & 0.963\\
 \hline
 15 & 26583.81 & 2359296 & 1.126 \\
 \hline
 18 & 5052.15 & 262144 & 1.927  \\

\end{tabular}
\caption{Effective number of parameters identified by our bound. Compression rates can be as low as $1\%$ in later layers (from 9 to 19) whereas earlier layers are not so compressible. Dependence on depth $d$, log factors, constants are ignored  as mentioned in the text.}\label{table:compress1}
\end{table}
